Bridge the Future: High-Performance Networks in Confidential VMs without Trusted I/O devices

Trusted I/O (TIO) is an appealing solution to improve I/O performance for confidential VMs (CVMs), with the potential to eliminate broad sources of I/O overhead. However, this paper emphasizes that not all types of I/O can derive substantial benefits from TIO, particularly network I/O. Given the obligatory use of encryption protocols for network traffic in CVM's threat model, TIO's approach of I/O encryption over the PCIe bus becomes redundant. Furthermore, TIO solutions need to expand the Trusted Computing Base (TCB) to include TIO devices and are commercially unavailable. Motivated by these insights, the goal of this paper is to propose a software solution that helps CVMs immediately benefit from high-performance networks, while confining trust only to the on-chip CVM. We present FOLIO, a software solution crafted from a secure and efficient Data Plane Development Kit (DPDK) extension compatible with the latest version of AMD Secure Encrypted Virtualization (SEV), a.k.a., Secure Nested Paging (SNP). Our design is informed by a thorough analysis of all possible factors that impact SNP VM's network performance. By extensively removing overhead sources, we arrive at a design that approaches the efficiency of an optimal TIO-based configuration. Evaluation shows that FOLIO has a performance dip less than 6% relative to the optimal TIO configuration, while only relying on off-the-shelf CPUs.

==> 1-intro.tex <==

\vspace{-5pt}
\section{Introduction}
\label{sec:intro}
Ensuring the security of cloud computation is essential for both cloud service providers (CSPs) and cloud users.
Trusted Execution Environment (TEE)~\cite{confidential_consortium:2022} is a popular hardware-based solution to secure cloud computation, offering a remote-measurable and trusted execution environment for cloud workloads.
Almost all major CPU vendors have TEE products, with a trend toward supporting confidential virtual machines (VM-based TEEs), including AMD Secure Encrypted Virtualization (SEV) series~\cite{kaplan:2017:seves,kaplan:2016:sevWpaper,amd:2020:snp}, ARM Confidential Compute Architecture (CCA)~\cite{arm:2021:cca}, and Intel Trust Domain Extensions (TDX)~\cite{intel:2020:tdx}. 
Moreover, major CSPs have launched commercial confidential-VM services enabled by AMD SEV, including Amazon AWS~\cite{aws:2023:sev}, Google Cloud~\cite{google:2020:sev}, and Microsoft Azure~\cite{microsoft:2021:sev}.

 
\subsection{Motivation: I/O Performance in the Next-Generation TEEs}
% Recent work has shown that I/O performance is a 
% in a virtualized environment can be a limiting factor 
% when deploying large-scale AI applications and other high-throughput applications in the cloud~\cite{zhao:2022:understanding, khan:2022:hvac}.
% \mengyuan{I change this sentence because we may not want to give a feeling that non-TEE VM is not fit for AI neither}
Recent studies highlight the critical role of optimal I/O performance in the deployment of large-scale AI and other high-throughput applications within the cloud environment~\cite{zhao:2022:understanding, khan:2022:hvac}. 
As TEE technologies introduce extra overhead due to their various security features, the poor I/O performance faced by TEEs~\cite{akram:2022:sok,akram:2021:performance} has raised even more critical concerns when designing next-generation TEEs.

\mengyuan{One unsolved part is that TIO is designed for all IOs, including disk and network. But we focus only on the network and DPDK is also a network-specific technique. So some logic maybe missing here.}

% Benefiting from the data protection provided by TEE, people are eager to deploy sensitive cloud workload inside confidential VMs, including large-scale AI models or high-throughput applications~\cite{confidential_consortium:2022}. 
% However, the relatively poor I/O performance becomes one of the primary reasons that hinder the adoption of confidential VMs~\cite{akram:2022:sok,akram:2021:performance}. 
% Several factors can count such performance degradation, including both overhead due to TEE-specific security design and common overhead due to virtualization. 

The industry has laid down a roadmap in obtaining high-performance I/O for confidential VMs.
Both Intel and AMD published whitepapers~\cite{intel:2023:tio,amd:2023:tio} to introduce specialized hardware devices, called trusted I/O devices (TIO), to remove the performance overhead associated with TEE-specific security features.
% , such as memory encryption and context switch overhead.
For example, 
% \replaced{
in existing confidential VM, a memory encryption technique~\cite{intel:2020:tdx,kaplan:2016:sevWpaper} is used to encrypt and protect the VM's memory, but it also introduces two performance drawbacks as well: (1) accessing memory requires decryption first, and (2) I/O devices cannot directly perform DMA operations on the VM's private memory, necessitating additional I/O data copying and encryption.
TIO mitigates such overhead by allowing the confidential VMs to establish a mutual trust relationship with TIO devices, so that they can securely share the memory encryption key and communicate directly using private memory.
% }{in existing confidential VMs, due to memory encryption~\cite{intel:2020:tdx,kaplan:2016:sevWpaper}, when an application attempts to send a network packet, the packet needs to go through a complex procedure, involving being first encrypted when writing to the memory, then being decrypted and re-encrypted using a different key before bypassed to the network device. TIO completely removes such overhead by allowing the confidential VMs to establish a mutual trust relationship with TIO devices, so that they can communicate directly using protected memory. By extending the trust boundary from the on-chip CPU to the peripheral device, TIO aims to achieve high performance matching a non-TEE setup.} 

\mengyuan{highlight DMA maybe more straightforward than encrypt/re-encrypt}



% To address the I/O bottleneck problem, the industry has a clear roadmap to tackle both overheads. To first solve the overhead due to TEE-specific security design, the industry is proposing a trusted I/O device (TIO) solution, which aims at extending the trust boundary from CPU side (VM-based TEE) to peripheral device side (device-based TEE) and achieving near non-TEE I/O performance.
% Both Intel TDX and AMD SEV recently released their TIO whitepapers~\cite{intel:2023:tio,amd:2023:tio} and the foundation behind the TIO solution is to enable confidential VM and trusted devices to share memory in a protected way. Specifically, in current confidential VM, a memory encryption technique~\cite{intel:2020:tdx,kaplan:2016:sevWpaper} is used to encrypt and protect the VM's memory, but it also introduces two performance drawbacks as well: (1) accessing memory requires decryption first, and (2) I/O devices cannot directly perform DMA operations on the VM's private memory, necessitating additional I/O data copying and encryption.
% With the help of TIO devices, a mutual trust relationship can be established between the I/O device and the confidential VM, enabling a secure sharing of the memory encryption key and mitigating most overhead due to TEE protection.

% \replaced{
Moreover, by extending the trust boundary from the on-chip CPU to the peripheral device, network I/O operations in confidential VM can now function similarly to a regular non-TEE VM. As a result, it can naturally benefit from other existing network techniques, such as Single Root I/O Virtualization (SR-IOV)~\cite{dong:2012:sriov} and Data Plane Development Kit (DPDK)~\cite{dpdk:2023:dpdk}. These techniques remove overhead due to virtualization and offer appealing network-boosting services.
Thus, we consider a futuristic configuration of confidential VMs that utilize TIO and incorporate the DPDK technique as an idealized setup, ultimately achieving the \textbf{\textit{idealized}} network performance.
% }{Moreover, after removing TEE-specific overhead, the plan goes with further improving the network performance via existing network techniques, such as Single Root I/O Virtualization (SR-IOV)~\cite{dong:2012:sriov} and Data Plane Development Kit (DPDK)~\cite{dpdk:2023:dpdk}.These techniques remove overhead due to virtualization and offer appealing network-boosting services.Thus, we consider a futuristic configuration of confidential VMs that utilize TIO and incorporate the DPDK technique as an idealized setup, ultimately achieving the \textbf{\textit{idealized}} network performance.}

% After eliminating the security boundary, the confidential VM can now function similarly to a regular non-TEE VM. As a result, it can naturally benefit from other existing network techniques, such as Single Root I/O Virtualization (SR-IOV)~\cite{dong:2012:sriov} and Data Plane Development Kit (DPDK)~\cite{dpdk:2023:dpdk}, to further mitigate overhead caused by virtualization and leverage full network boosting services, ultimately achieving the \textbf{\textit{Idealized}} network performance.

% As suggested by the whitepaper, when used in conjunction with Single Root I/O Virtualization (SR-IOV)~\cite{dong:2012:sriov}, TDISP allows the NIC to virtualize different device virtual functions (VFs) and treat each VF as an independent TEE device interface (TDI)~\cite{intel:2023:tio} assigned to one VM. Subsequently, this VM can operate like a traditional VM without TEE protection and further benefit from any other network techniques, including Data Plane Development Kit (DPDK)~\cite{dpdk:2023:dpdk}. This allows the VM to achieve end-to-end network optimization, high-performance network processing, and meet the demands of enterprise-level applications.  

% The future idealized solution.


% that certain specialized I/O devices themselves can be considered as trusted device-based TEEs. Once a mutual trust relationship is established between the trusted device and the confidential VM through the TEE Device Interface Security Protocol (TDISP)~\cite{amd:2023:tio,intel:2023:tio}, the trusted device can share the memory encryption key with the confidential VM, thereby gaining direct access to the encrypted private memory within the VM.




% The cumulative extra network overhead caused by different TEE protection mechanisms could be a fundamental factor limiting the ability to run large-scale AI models or high-performance computing in a confidential VM configuration.



% To solve the I/O bottleneck problem in confidential VMs, the industry is proposing trusted I/O device (TIO) solution, which aims at extending the trust boundary from CPU side (VM-based TEE) to peripheral device side and achieving trusted high-performance I/O.
% To achieve large network throughput and minimal network latency, Intel recently introduced Intel TDX Trusted I/O~\cite{intel:2023:tio}, and AMD SEV also recently published the TIO whitepaper~\cite{amd:2023:tio} for high-performance network communication. 
% The foundation behind TIO solution is that certain specialized I/O devices themselves can be considered as trusted device-based TEEs. Once a mutual trust relationship is established between the trusted device and the confidential VM through the TEE Device Interface Security Protocol (TDISP)~\cite{amd:2023:tio,intel:2023:tio}, the trusted device can share the memory encryption key with the confidential VM, thereby gaining direct access to the encrypted private memory within the VM.


% the TEE Device Interface Security Protocol (TDISP)~\cite{amd:2023:tio,intel:2023:tio}, proposed together by CPU vendors, PCI Special Interest Group (SIG), and other industry partners. With the assistance of a trusted device security module (DSM) on the device side, TDISP defines how to establish a trusted relationship between confidential VMs and TEE I/O compliant devices. TDISP enables authenticated TEE I/O devices to directly access the confidential VM's private memory and ensures confidentiality and integrity protection for the corresponding data streams within PCIe. 

% The support for trusted I/O devices can solve this problem naturally. In the case of Single Root I/O Virtualization (SR-IOV)~\cite{dong:2012:sriov} capable devices, TDISP allows each I/O device virtual function (VF) to act as an independent TEE Device Interface (TDI)~\cite{intel:2023:tio} and gain direct access to the private memory of the confidential VM using the VM's memory encryption key after authentications. 

% \paragraph{Problems}
Though promising, the TIO technology exhibits several limitations.
First, we face the problem that the community cannot benefit from TIO before they are commercially available.
Due to the lengthy hardware product cycles, it usually takes years for new hardware technology to be widely accessible.
% Given that the promotion of TIO technology requires close coordination with the development of interface standards, its  is unpredictable 
For example, the Intel TDX whitepaper was published in 2020, but commercial CPUs supporting it are not yet available at the time of writing. 

Second, the TIO technology expands the Trusted Computing Base (TCB) of a system to include peripheral devices.
The original TCB of existing TEEs is enclosed inside a monolithic chip.
% \mengjia{correct?}. \mengyuan{Yes}
With TIO, the overall security of the TEE will be contingent upon the weakest link between the TIO devices and the CPU-based TEE. 
Thus, the TIO technology poses research challenges to verify the security properties of a complex and heterogeneous system, which by itself may take time to fully examine by industry and academia.
% is an unsolved research problem for the industry and academia.


% Even though such idealized solution presents a promising future for next-generation TEEs, there are two major reasons why our community might not immediately benefit from it: (1) it may take years to make TIO devices available considering the lengthy hardware product cycles. For example, the Intel TDX whitepaper was published in 2020, but commercial CPUs supporting it are not yet available at the time of writing. 
% (2) TIO solution can introduce trusted computing base (TCB) as it has unique threat models where TIO devices are also trusted. As a result, the overall security of the confidential VM is contingent upon the weakest link between the TIO devices and the CPU-based TEE. Directly extending trust to TIO devices is risky since evaluating the security of their design thoroughly requires time and efforts from both the industry and academia.

% \mengjia{so to summarize our situation: the trusted IO devices are not here yet, how can we boost the performance of IO devices given all the performance need?}


Given the above concerns related to TIO technology, this paper aims to enable confidential VMs to immediately benefit from high-performance network I/O without relying on TIO.
Specifically, we explore a solution that can achieve the same level of I/O performance as the idealized confidential VM setup, and offer the same security guarantees as existing confidential VMs, where the TCB is enclosed within the on-chip TEE-based CPUs.
As we offer a secure and efficient network solution, our solution serves as a \textit{bridge} toward the future idealized solution.


% Therefore, this raises the research question that our paper focuses on:
% \vspace{6pt}
% \begin{center}
% \minibox[rule=1pt,pad=2pt]{
% \begin{minipage}[h]{0.9\columnwidth}
% {\it \textit{
% Is it possible to achieve the same level of I/O performance without trusted I/O devices and sacrificing the existing security guarantees?}}
% \end{minipage}
% }
% \end{center}
% \vspace{7pt}
% We believe that exploring how existing untrustworthy network devices and software solutions can achieve high-speed and secure communication in confidential VMs will remain highly valuable in the coming years, serving as a crucial \textit{bridge} towards the future idealized solution. 
% To bridge the future, where SR-IOV and DPDK will be extensively utilized by the TIO devices to enable high-performance I/O, our research objective is to keep the secrets of confidential VMs within the CPU TEE side and achieve high-performance I/O while maintaining the same level of security as the default VirtIO~\cite{russell:2008:virtio} used by current confidential VM. 
% \mengjia{Is it possible to avoid the jargons in this sentence but still express yourself clearly, such as SR-IOV, DPDK, VirtIO? }


% \mengjia{first, this is a really long sentence; second, DPDK deserves a brief explanation.}

% \subsection{Comprehensive Analysis of I/O Performance Overhead Sources}
\subsection{\sysname: Secure and Performant DPDK extension for SNP VMs}


This paper presents \sysname, a software solution that enables a secure and efficient DPDK extension compatible with confidential VMs.
Our design is driven by a comprehensive analysis that thoroughly investigate the factors that can influence network performance in confidential VMs.
Specifically, we study the network performance of the latest version of AMD SEV (SEV-SNP), the only commercially available confidential VM at the time of writing. 


% To address the overhead in the current SEV-SNP network I/O solution, 
% we first conducted a series of exploratory experiments to thoroughly investigate the factors influencing network performance. These factors encompassed both factors due to SEV-specific protections and common factors introduced by virtualization.

We classify the network overhead sources into two major categories, either due to virtualization or TEE-specific security features.
Our analysis leads to two insightful discoveries.
First, the routing overhead of virtualization is the dominant factor across all overhead sources, while the TEE-specific overhead plays a marginal role.
As TIO focuses on removing TEE-specific overhead, we are motivated to think about the possibility of reducing the gap with the idealized network performance without TIO support.

Second, by enumerating and comparing the overhead sources of a designated software-only DPDK-supported design and the idealized design, we find the only difference lies in the additional memory copy overhead, which merely accounts for less than 2\% of tail latency.
This overhead is unavoidable in a software-only solution because the network device cannot directly communicate with the guest application via shared memory.
This discovery further strengthens our confidence about the possibility of \textit{closing} the gap (rather than just reducing the gap) with the idealized network performance for confidential VMs.

% The experiment results indicate that memory encryption and other SNP-induced protections are not the primary factors contributing to the subpar network performance in SNP-enabled VMs. 
% Instead, the predominant bottleneck, accounting for more than 50x of the performance degradation, stems from the latency introduced by emulated I/O device in the virtualized environment.
% By leveraging SR-IOV technology, such overhead can be bypassed. 
% \mengjia{Do not think it is important to mention in the intro.}

% Another interesting observation is that the overhead introduced by memory copy may be less than 2\%. This finding gives us hope that even without TIO devices, we can potentially achieve similar I/O performance compared to the future idealized solution. By collaborating with DPDK to address most influencing factors related to SEV-specific protections and further minimize the overhead caused by memory encryption, we can reduce all overhead to the greatest extent with software-only solutions.
% However, due to memory encryption, SNP VMs cannot directly benefit from DPDK without TIO devices. Instead, DPDK's specific optimizations may expose additional information to the hypervisor or allow the hypervisor to compromise the integrity of existing DPDK applications.

% \mengjia{I think I understand S1.1 and S1.2. Just need to polish the text to make the writing more fluent.}
% To further reduce the overhead caused by SNP's protection, such as the overhead from SNP's register protection ($\sim$10\%) and the overhead from emulated interrupts and user-kernel space routing within the VM (>2x), how to avoid these events from causing extra overhead in the SNP becomes essential. Surprisingly, if DPDK can be safely and efficiently supported in the SNP configuration, all known factors can be minimized as much as possible, except for one additional I/O data copy, which our experiments indicates may have only a less than 2\% impact. This observation gives us hope that even without TIO devices, we may still be able to achieve similar I/O performance compared to the idealized solution using software-based methods.


We then design \sysname, short for Fast, Optimized, Locked (protected) I/O.
\sysname is a DPDK-based software solution specifically designed for AMD SEV-SNP.
The goal of \sysname is to achieve network I/O capabilities matching the future idealized solution with TIO support, including both performance and functionality, while confining trust only to the on-chip CPU TEE. 



% In this paper, we proposed a DPDK-based software solution specifically designed for AMD SEV-SNP, 
% % called Confidential Userspace Rapid I/O (\sysname), 
% called Fast, Optimized, Locked (protected) I/O (\sysname), 
% which carefully deal with private and shared memory and achieves the same end-to-end security level as the default VirtIO solution used in current SNP VMs. 
% \mengjia{the private and share memory problem was not discussed.\\
% An attempt below:
% To make DPDK compatible with AMD SEV-SNP, we face the security challenge described below.
% In DPDK, we aim to make the user-level application to directly communicate with the network device, so that we can bypass substantial overhead due to virtualization.
% Howeover, following the TEE threat model, the user-level application cannot directly place its data (packet, metadata, etc) in a shared region that is accessible to the network device.
% Because the shared region is broadly accessible by the malicious host hypervisor and we end up suffering from serious confidentiality and integrity problems.
% As such, we need a mechanism to carefully deal with the data communication issue by coordinating the data management of the shared memory.\\
% (I feel private memory is not important, the problem is due to shared memory leak too many things... you use private memory as a solution. To make it more clear: The problem arises due to shared memory can be accessed/manipulated by anything; Your solution is to use the private memory as a shadow region...)}

% \mengjia{I like this sentence.}
% \mengjia{can you explain our scheme without DPDK? Is DPDK kernel bypass. So will the following statement be correct: our scheme leverages guest kernel bypass to significantly remove/eliminate routing overhead. We design the guest kernel module to interact with the potentially malicious host using shadow memory to achieve the same level of security as ....}

% \mengjia{check this paragraph.}
To achieve this goal, \sysname meticulously manages two interfaces: the one between the I/O device and the confidential VM, and the one between the DPDK library and the DPDK application.
We introduce shadow memory to coordinate the secure communication over shared memory between the DPDK application and the I/O device.
% This approach guarantees the security of both the VM and existing DPDK applications while maintaining source code compatibility, secure memory management, and minimizing network overhead.
Additionally, \sysname provides network-boosting functionalities, such as packet encryption offloading, using on-core computation resources.
We offer comparable performance with future TIO solutions without expanding the TCB of our system.
% Additionally, \sysname offers extra functionalities that may be potentially supported in TIO solution, such as packet encryption offloading. 



We evaluate the performance benefits of \sysname compared to existing confidential VM configurations under different network loads.
Furthermore, we estimate the performance gap between \sysname and the idealized TIO and DPDK combination.
Limited by the unavailability of TIO devices, we cannot directly obtain the idealized performance number.
Alternatively, we conservatively consider the idealized combination can achieve network performance for a non-TEE configuration.
Our extensive experiment results show that the gap between \sysname and the future idealized configuration is no more than 6\% in tail latency.


% The performance of \sysname is evaluated under different network loads, and we also compare the performance difference between \sysname and future idealized solution in an estimated manner.
% Experimental results indicate that \sysname should incur no more than 6\% network overhead across various network workload intensities compared to future idealized solution relying on TIO devices. Moreover, the generic design solution proposed by \sysname can be easily extended to other confidential VM platforms. 

The contributions of our work are summarized as:
% follows:

\begin{packeditemize}

\item This paper investigates the impact of additional protections introduced by AMD SEV series on network performance and provides a detailed analysis of how confidential VMs may address these overheads.

\item This paper proposes a DPDK-based network solution (\sysname) tailored for SNP VMs, which achieves high-speed network performance comparable to the future idealized TIO solution without compromising existing I/O security. 
% This is achieved by restricting the interfaces between VMs and I/O devices and the interfaces between DPDK library and DPDK applications. The system also supports crypto operations offload and ensures source code compatibility.

\item This paper evaluates the performance of \sysname and estimates the performance difference between \sysname and future idealized solution. Experimental results indicates the estimated performance difference is within 6\%.

\item This paper enhances an existing DPDK measurement tool to support end-to-end IPsec traffic measurement in the context of confidential VM environment.

\end{packeditemize}

% \bheading{Paper outline.} The rest of the paper is organized as follows: \secref{sec:background} introduces background information about confidential VM and AMD SEV, as well as relevant network techniques; \secref{sec:motivation} and \secref{sec:conclusion} concludes the paper.

% In the paper, we aim to answer the following research questions:
% \begin{enumerate}[label=\textbf{Q\arabic*.}]
% \item \label{q1} What are the network performance bottlenecks of SEV-SNP enabled VMs?
% \item \label{q2} How is network I/O security ensured in SEV-SNP enabled VMs?
% \item \label{q3}
% Without a trusted I/O device, what is the performance limit of network I/O in SEV-SNP enabled VMs while ensuring security?
% \item \label{q4} What optimizations can Trusted I/O device bring?
% \end{enumerate}

==> 11-notes.tex <==
\section{Notes}
\label{sec:notes}
The research questions we want to answer in this paper include
\begin{enumerate}[label=\textbf{Q\arabic*.}]
\item \textbf{Performance.}\label{rq1} 
\item \textbf{Security.}\label{rq2} 
\end{enumerate}

==> previous_review.tex <==
\newpage
\newpage
\newcommand{\rebut}[1]{\textcolor{blue}{\bf Response: #1}}
\section*{Executive Summary}
\added{This paper was previously submitted to IEEE S\&P 2024. We greatly appreciate the constructive feedback provided by the previous reviewers, who are all experts in our TEE research community. Their main suggestions have been summarized as follows:}

\vspace{3pt}
\begin{center}
\begin{minipage}[h]{0.95\columnwidth}{
\begin{packeditemize}
\item First part doesn’t provide deep insights (Reviewer A \& B)
\item First part has some imprecise parts (Review A)
\item The consequence of the design choice is not well discussed (Review A \& B)
\item Two parts seem to be disconnected (Reviewer A \& B)
\item The second part is just a very initial exploration of using an operational model to analyze TEEs (Reviewer A \& B)
\end{packeditemize} }
\end{minipage}
\end{center}
\vspace{3pt}

\added{These feedbacks are immensely helpful in the revision. Given the multitude of existing TEE designs with different design considerations, conducting a systematization of knowledge specific to TEE runtime poses significant challenges. Consequently, there may have been inadvertent omissions or imperfect expressions in our original version. With the structural feedback and detailed suggestions given by the previous reviewers, we have made the following improvements to the paper. We also wholeheartedly welcome further suggestions to enhance this paper and potentially attract more researchers to focus on and contribute to the field of confidential computing.}

\bheading{Revision Summary:}

\bheading{Clarify the motivation.} In response to the reviewer's feedback, we have clarified the motivation of our paper in the introduction section. The high-level part (TRAF) aims to provide new researchers with a systematic and efficient approach to deconstructing a TEE design, assisting them in choosing a research direction of interest. The low-level part (TRAM) delves into a TEE design from a microarchitectural perspective, which could be helpful in establishing a deep understanding of a specific TEE and aiding researchers in exploring potential security vulnerabilities.
% \yuheng{arch-level and microarch-level -> high/low-level}

\bheading{Add consequences of design choices.} We have added the consequences of design choices in Section 4 to highlight the impact and implications of different design decisions. This addition enhances the comprehensiveness of our analysis.

\bheading{Address imprecisions and mistakes.} We have carefully addressed all known imprecise parts accordingly. The reason for not considering embedded TEE designs was due to our previous lack of clear description. We explicitly focus on server-side TEEs in our study.

\bheading{Explain the connection and motivation.} We have added the connection and motivation of including the deconstruction frame and the operational model in Section 4. 

\bheading{Expand TRAM model.} We have expanded the TRAM sections with additional details, including descriptions of other attack scenarios and clarifications where necessary. Additionally, we have formally modeled Keystone and Penglai as two additional examples in TRAM. However, it is important to emphasize that the motivation behind TRAM is to accurately describe the low-level implementation of a TEE design from a microarchitectural perspective. The main focus of TRAM is on the procedures of modeling, which should plays a helpful role for researchers to understand TEE implementation details. Our primary focus is not solely on modeling all existing TEE designs by ourselves, which limits the our original intention.

\section*{Previous Reviews (IEEE S\&P 2024)}
An unaltered copy of previous review is provided below for reference purposes:

\subsection*{\textcolor{Maroon}{Review A}}

\bheading{Paper summary:}
This paper addresses the problem of efficient network IO with confidential VMs. More specifically, it proposes a framework based on DPDK and SR-IOV with confidential VMs without the need for trusted IO devices or the related infrastructure for attestation (e.g., TDISP). The proposed solution limits the TCB to just the CPU (and requires no trust in the device). The authors claim that the overhead compared to the ideal trusted IO setting (with enlightened devices + SRIOV in a confidential VM), their solution FOLIO may have an overhead of upto 6\%.

The paper includes a detailed analysis of the overheads incurred during IO operations for confidential VMs (and quantifies them). It also includes a prototype implementation of the solution and comparison with a non-TEE VM + SRIOV.

\bheading{Technical Correctness:}
3. Fixable Major Issues

\bheading{Technical Correctness Comments:}
The only concern I have in terms of technical correctness is the extrapolation of the performance results to compare to non-existent TIO solutions/devices. It's fine to speculate about how the performance might compare but, the conclusions in the paper aren't obvious to me. E.g.. the paper is missing discussion on major sources of overhead for TIO such as the link protection but it is not clear why that is so. I know that it doesn't help the TIO case (maybe FOLIO comes off better?), but that doesn't make the paper any more complete.

In table 1, the only sources of overhead of TEE+TIO over non-TEE+DPDK is a bounce buffer copy + ownership check overhead --> both of which the authors claim are not significant. But the authors claim that there will be a significant difference in performance between the two in section 5.

\bheading{Scientific Contribution:}
7. Establishes a New Research Direction

\bheading{Scientific Contribution Comments:}
1. The paper offers a systematic study of various sources of overhead for IO in virtualized systems in general and confidential VMs in particular (although some aspects are unclear/missing - see below). The part about the bounce buffer being small overhead is an interesting result.
2. The paper presents an entire framework and prototype for improving the performance of networking applications with SEV-SNP without the need for costly and yet-to-be available trusted IO devices. This is done at the cost of extra memory, potentially additional CPU threads for crypto acceleration.
3. The paper reduces the trust boundary of the trusted IO solution to the CPU socket boundary; while not generic, it is still an impressive achievement for an important application esp. since it is significantly better in performance than the baseline (TEE+emulated IO).

\bheading{Presentation:}
2. Minor Flaws in Presentation

\bheading{Presentation Comments}
There are a few places in the paper which require a scrub for consistency/clarity.

E.g., In section 6, the paper claims that a Non-TEE VM will surpass the perf. of a TEE VM+ TIO because the former avoids a bounce buffer. Doesn't the latter avoid a bounce buffer too? Besides, didn't the authors conclude that the bounce buffer is not really the major source of overhead?

E.g., why is there a need for SW-based encryption to prevent potential  leakage during network routing (section 7.1)? What is this leakage and how does encryption solve a routing leakage problem?

E.g., Throughout the paper, I see a mention of SEV memory encryption as a source of overhead and yet, I don't fully grok what the authors are referring to. Is it the fact that bounce buffers tend to use different memory encryption keys than the SEV-VM private memory and re-encryption is required? But all this memory is cacheable, and there is a way to make the shared memory unencrypted --> so, ideally the memory overhead seems orthogonal to the problem. Could the authors clarify what they mean?

E.g. could you rank the sources of overhead from largest to smallest in Table 1.

E.g., the columns of SEV, SEV-ES is really moot except to understand SEV-SNP better.


\bheading{Comments to Authors:}
Thank you for a well-written and data-driven analysis of the overheads in network virtualization for confidential VMs. The paper was a pretty good read and the results are quite educational.

Below are a few things to consider in terms of the practicality of FOLIO once trusted IO devices are available.
1. While we say that the overall memory requirements for networking buffers doubles with FOLIO, I didn't see a number attached to the typical sizes of the buffers? I'd recommend putting that into a table just to understand how it sizes up against the size of the VM memory itself.

2. The scheme in the paper only works for TIO in the case of specific types of workloads that typically don't require processing by the device itself, i.e., for pass-through devices.
- The crypto-acceleration offload to the CPU really takes away from the actual goal of the acceleration in the first place - to save costly CPU cycles and use cheaper accelerator cycles. Besides, the cost of an entire CPU thread just to perform inline crypto is not really an option; often that means including/paying for an entirely extra thread/vCPU.
- Accelerators are likely to get smarter over time even for networking (e.g., smart NICs/DPUs/IPUs) --> there is plenty of functionality that is unlikely to move back to the CPU. So, while solutions like FOLIO can handle specific acceleration functionality like crypto thanks to the availability of such hardware in the CPU, it is unlikely a popular mode of operation once trusted IO devices are available.
- why don't the optimizations for efficient I/O event handling application to TIO? Also, isn't it true that TIO doesn't require a copy before processing and shadow buffer pool usage? More generally, why don't the FOLIO optimizations for routing within a VM, within host applicable to TIO?

3. While it seems fair to compare the performance of TEE VM+FOLIO with a baseline of non-TEE+SRIOV+DPDK, it is really not clear how the authors make any claims w.r.t. TEE-VM + TIO. The statements in section 6 seem like a guess at best and is predicated on hardware vendors not optimizing the routing behavior for network packets for IO (e.g. using trusted interrupts and efficient routing). It would be better not to speculate about what cannot be measured or at least clarify the assumptions around that speculation.

4. The authors miss a very large source of overhead in industry directions for trusted IO in confidential VMs - the link protection overhead. It is worth adding this to the discussion in the paper. It is unclear if they disregarded this due to the network packets already being cryptographically protected. Please clarify.

5. Could you say if there is something specific about the design of SEV-SNP that helps/hurts FOLIO? What would change if FOLIO was to be used with TDX/CCA? How would the perf. gains against the baseline compare?

\bheading{Recommended Decision:}
3. Weak Reject (Can be Convinced by a Champion)

\bheading{Reviewer Confidence:}
2. Highly Confident

\bheading{Should this submission be reviewed by the Research Ethics Committee?}
1. No

\subsection*{\textcolor{Maroon}{Review B}}
\bheading{Paper summary:}
This paper aims to enable confidential VMs to have high-performance I/O without depending on TIO. The proposed system called Folio, a software solution crafted from a secure and efficient DPDK extension with AMD SEV-SNP. The  proposed approach removes the performance overhead sources, and provides a TIO-driven solution, incurring additional overhead only from a single memory copy. The evaluation results show that Folio has a less than 6\% performance dip relative to the idealized TIO solution.

\bheading{Technical Correctness:}
1. No Apparent Flaws

\bheading{Technical Correctness Comments:}
I feel there is no apparent flaws on technical correctness.

\bheading{Scientific Contribution:}
6. Provides a Valuable Step Forward in an Established Field

\bheading{Scientific Contribution Comments:}
This paper combines DPDK with SEV for achieving a secure and fast IO.

\bheading{Presentation:}
1. No Flaws in Presentation

\bheading{Presentation Comments}
I think no major presentation issues for this paper.


\bheading{Comments to Authors:}

Strengths:

+ Improving the IO performance of Secure Virtual Machines is important.

+ Good combination between SEV and DPDK.

+ The evaluation shows that the proposed approach can improve the IO performance of SEV.

Weaknesses:

- The technical challenges of applying DPDK on SEV are not clear to me.

- The security impact on shared buffer needs to be justified.

- The approaches used for constrained DPDK-APP interfaces are straight-forward.

Detailed Comments:

This paper aims to improve the performance of the secure virtual machines. In particular, this paper focuses on AMD SEV. I agree that the improving the IO performance is important for secure VMs. This paper combines SEV and DPDK to achieve the goal. The evaluation shows a promising IO performance results.

The first question that I have for this paper is: what improves the IO performance of AMD SEV. If I understand correctly, the DPDK itself was intended to speed up the IO performance. I feel that this paper shows a simple combination of DPDK and SEV. It might be better if the paper can highlight the technical changes to combine DPDK and SEV for improving the performances.

Constrained VM-I/O interaction interfaces. This is mainly designed for achieving the security purpose. However, it is to clear to me how to ensure the security of the data in the shared memory such as the memory location, length, or status of network packets. What if a malicious modify the meta data of the network packets? Will it compromise the security of IO operations?

Constrained DPDK-APP interaction interfaces. To achieve this goal, this paper proposed several techniques including 1) copy before processing, 2) shadow packet buffer pool, and 3) conceal shared region and fault handing. Copy before processing is trivial for security; and the other two techqniues are straight-forward to me.

As the paper mentions that network applications without DPDK support cannot benefit from Folio. I feel that this might be a limitation of the proposed approach since the scope of the application might be restricted.


\bheading{Recommended Decision:}
3. Weak Reject (Can be Convinced by a Champion)

\bheading{Reviewer Confidence:}
2. Highly Confident

\bheading{Should this submission be reviewed by the Research Ethics Committee?}
1. No

==> x-intro-backup.tex <==
\section{Introduction}
\label{sec:intro}
% \begin{verbatim}
% In introduction, we talk about 
% (1) the trend for confidential computing and 
%     the trend for confidential VM instead of enclave, 
% (2) Two concerns about CVM, one is its security, 
%     since the boundary is boarder, 
%     The second concern is the performance, especially 
%     for high performance computing -> cite papers
% (3) briefly mention that Intel/AMD proposed TIO, 
%     but because of its long circle 
%     and hardware device support. 
%     It may still need years to be deployed
%     So We aim to explore the reason behind 
%     and perform a comprehensive study 
%     of its performance bottlenecks
% (4) Research questions
% (5) Contributions. 
% (6) Roadmaps
% \end{verbatim}


The security of cloud data is a critical concern that deters many potential cloud users from adopting cloud services. Consequently, addressing the challenge of ensuring the security of cloud workload can create a mutually beneficial situation for both cloud service providers (CSPs) and cloud users. Trusted Execution Environment (TEE)~\cite{confidential_consortium:2022}, as a hardware-based solution of this challenge, provides a remote-measurable and trusted computing environment with significant performance advantage compared to cryptographic-based solution, such as homomorphic encryption~\cite{van:2010:homomorphic}. By confining the Trusted Computing Base (TCB) to the delicate System-on-Chip (SoC) and limited hardware-protected software stacks, TEE ensures the confidentiality and integrity of cloud workload. 
% \mengjia{delicate? I thought delicate implies something is easy to be broken, but you want to say it offers strong security right?}\mengyuan{I want to say soc is tiny so hardware attacks are hard.}
Naturally, such approach has garnered attention from both the industry and academia since the introduction of TEE. Regarding the numerous existing TEE designs, they can generally be categorized into enclave-based TEEs (\eg Intel Software Guard Extensions (SGX) ~\cite{van:2017:sgx}, RISC-V Keystone~\cite{lee:2020:keystone}, Penglai~\cite{feng:2021:penglai}) and VM-based TEEs (\eg AMD Secure Encrypted Virtualization (SEV) series~\cite{kaplan:2017:seves,kaplan:2016:sevWpaper,amd:2020:snp}, ARM Confidential Compute Architecture (CCA)~\cite{arm:2021:cca}, and Intel Trust Domain Extensions (TDX)~\cite{intel:2020:tdx}). 

\subsection{Motivation: I/O Performance in Next-Generation TEEs}
% It is worth mentioning that there are two noticeable trends in the field of industrial TEE designs. The first trend is that the industry has shifted its focus from enclave-based TEE to VM-based TEE. This is evident in Intel's decision of discontinuing SGX support for desktop-level processors~\cite{intel:2022:discontinue_sgx} and the emergence of commercial confidential VM designs from major CPU vendors recent years, including AMD SEV (2017), Intel TDX (2020), and ARM CCA (2021). 
Compared to enclave-based TEEs, VM-based TEEs leverage the entire VM as their security boundaries, enabling the execution of trusted programs at different scales without the need for source code modifications and better performance. 
At the time of writing, major cloud providers have launched commercial confidential VM services enabled by AMD SEV, including Amazon AWS~\cite{aws:2023:sev}, Google Cloud~\cite{google:2020:sev}, and Microsoft Azure~\cite{microsoft:2021:sev}. 

However, even VM-based TEEs encounter network I/O challenges~\cite{akram:2019:using,akram:2022:sok,akram:2021:performance,chen:2023:confidential}. The additional protection introduced by TEE for various events or instructions may result in varying degrees of overhead on network performance. 
For example, memory encryption is a common protection mechanism used in confidential VMs, but it introduces two performance drawbacks as well: (1) accessing memory requires decryption first, and (2) I/O devices cannot directly perform DMA operations on the VM's private memory, necessitating additional I/O data copying and encryption. 
The cumulative extra network overhead caused by different TEE protection mechanisms could be a fundamental factor limiting the ability to run large-scale AI models or high-performance computing in a confidential VM configuration.

The support for trusted I/O devices can solve this problem naturally. In the case of Single Root I/O Virtualization (SR-IOV)~\cite{dong:2012:sriov} capable devices, TDISP allows each I/O device virtual function (VF) to act as an independent TEE Device Interface (TDI)~\cite{intel:2023:tio} and gain direct access to the private memory of the confidential VM using the VM's memory encryption key after authentications. 


% These trends reflect the cloud community's demand for large-scale, high-performance confidential computing. Compared to traditional VMs, the additional protections added by TEE design seem to cause non-negligible I/O performance overhead. 

% \mengjia{Suggest adding 1-2 paragraphs on how \textbf{important} IO performance matters nowadays in cloud computing. Such as tail latency, network device speed going up and many packets need to be processed per seconds, etc.}


% \mengjia{I have a problem with the following discussion: the discussion below does not provide a clear picture of the current state of IO techniques and performance in TEE VMs. 
% Can you provide a describe of where we are and what problem we have without those trusted IO devices?}

The second trend is that the industry is proposing trusted I/O devices, which aims at extending the trust boundary from CPU side (VM-based TEE) to peripheral device side and achieving trusted high-performance I/O.
As a prerequisite for large I/O throughput server applications or AI training, Intel recently introduced Intel TDX Trusted I/O~\cite{intel:2023:tio}, and AMD SEV also recently published the TIO whitepaper~\cite{amd:2023:tio} to achieve high-performance network communication. 
The foundation behind trusted I/O devices is the TEE Device Interface Security Protocol (TDISP)~\cite{amd:2023:tio,intel:2023:tio}, proposed together by CPU vendors, PCI Special Interest Group (SIG), and other industry partners. With the assistance of a trusted device security module (DSM) on the device side, TDISP defines how to establish a trusted relationship between confidential VMs and TEE I/O compliant devices. TDISP enables authenticated TEE I/O devices to directly access the confidential VM's private memory and ensures confidentiality and integrity protection for the corresponding data streams within PCIe. 



However, it is uncertain whether our community can immediately benefit from trusted I/O devices. Considering the hardware dependencies of TEE solutions, their product cycles tend to be lengthy (the Intel TDX whitepaper was published in 2020, but commercial CPUs supporting it are not yet available at the time of writing). Additionally, trusted I/O devices introduce unique threat models where trusted I/O devices are included in the trusted computing base (TCB). As a result, the overall security of the confidential VM is contingent upon the weakest link between the trusted I/O devices and the CPU-based TEE. It is risky to directly extend trust to Trusted I/O devices because evaluating the security of their design thoroughly requires time and efforts from both the industry and academia. 

\mengjia{so to summarize our situation: the trusted IO devices are not here yet, how can we boost the performance of IO devices given all the performance need?}
Therefore, this raises the research question that our paper focuses on:
\vspace{6pt}
\begin{center}
\minibox[rule=1pt,pad=2pt]{
\begin{minipage}[h]{0.9\columnwidth}
{\it \textit{
Is it possible to achieve the same level of I/O performance without trusted I/O devices and sacrificing the existing security guarantees?}}
\end{minipage}
}
\end{center}
\vspace{7pt}
we believe that exploring how existing untrustworthy network devices can achieve high-speed and secure communication in confidential VMs will remain highly valuable in the coming years, serving as a crucial \textit{bridge} towards future trusted I/O devices. To bridge the future, where SR-IOV and Data Plane Development Kit (DPDK) will be extensively utilized by the trusted I/O devices to enable high-performance I/O, our research objective is to keep the secrets of confidential VMs within the CPU TEE side and achieve high-performance I/O while maintaining the same level of security as the default VirtIO~\cite{russell:2008:virtio} used by current confidential VM. 
\mengjia{first, this is a really long sentence; second, DPDK deserves a brief explanation.}
Specifically, this paper focuses on the network performance of the widely adopted AMD SEV-SNP, which is the only commercial available confidential VM at the time of writing. 

\subsection{Comprehensive analysis of SEV's diverse security protection measures and their impact on network performance.}

\subsection{This Paper: Secure and performant DPDK extension for confidential VM}
% minimize these overheads an

\mengjia{the first sentence reads as if those efforts were conducted by other people, not this paper....}
A series of efforts have been made to achieve this objective. These efforts include:
(1) To address the overhead in the current SEV-SNP network I/O solution, we first conducted a series of exploratory experiments to investigate the impacts of the additional protections incorporated into the AMD SEV-SNP design on network performance. The experiment results indicate that memory encryption and other SNP-induced protections are not the primary factors contributing to the subpar network performance in SNP-enabled VMs. Instead, the predominant bottleneck, accounting for more than 40x of the performance degradation, stems from the intricate routing latency introduced by I/O virtualization within the VM and on the host side. 
\mengjia{the term routing is not explicitly defined. Is this a widely used common term for the security community? Routing can also be related to network routing.}
By leveraging SR-IOV technology, the overhead due to routing on the host side can be bypassed. However, the DPDK support for SEV-SNP is currently unavailable, which is essential to eliminate the routing overhead within the VM.
(2) We achieved a DPDK implementation specifically for confidential VM setup, which carefully deal with private and shared memory and achieves the same security level as the default VirtIO. This implementation retains source code compatibility, secure memory management, and minimizes network overhead. [To add more details]. A security analysis showing our system does not downgrade the security level is also included.
(3) We have estimated the performance difference between our system and future trusted I/O solutions. Experimental results indicate that our system incurs no more than 6\% overhead across various network workload intensities compared to future systems relying on trusted I/O devices.
% \vspace{6pt}
% \begin{center}
% \minibox[rule=1pt,pad=2pt]{
% \begin{minipage}[h]{0.9\columnwidth}
% {\it \textit{What are the network performance bottlenecks of SEV-SNP enabled VMs?}}
% \end{minipage}
% }
% \end{center}
% \vspace{7pt}

% Our series of in-depth experiments indicate that memory encryption and other protection introduced by SNP are not the main causes of poor network performance in SNP-enabled VMs. Instead, the performance bottleneck primarily (more than XX\%) arises from the complex routing latency introduced by I/O virtualization, which is an old problem in virtualization. With the help of SR-IOV technology, routing at the host kernel level can be bypassed, resulting in a performance improvement of several orders of magnitude for SNP VMs as well. To achieve truly high-performance network computing, bypassing guest VM kernel-level routing is crucial. However, DPDK is not supported in SNP VMs, so the second research objective of this paper is:

% \mengjia{It does not sound like to be a good idea to mention DPDK directly without providing more context.}


% Thus, we also propose the third research question in this paper:
% What is the difference between XX(our implementation) and the trusted I/O device solution in terms of security and performance?



% \vspace{6pt}
% \begin{center}
% \minibox[rule=1pt,pad=2pt]{
% \begin{minipage}[h]{0.9\columnwidth}
% {\it \textit{What is the difference between XX(our implementation) and the trusted I/O device solution in terms of security and performance?}}
% \end{minipage}
% }
% \end{center}
% \vspace{7pt}


The contributions of this paper are summarized as follows:

\begin{packeditemize}

\item This paper investigates the impact of additional protections introduced by AMD SEV series on network performance and provides a detailed analysis of how confidential VMs can address these overheads.

\item This paper proposes a DPDK-based system (\sysname) adapted for SNP VMs, achieving high-speed network communication without compromising existing I/O security. This is achieved by restricting the interfaces between VMs and I/O devices and the interfaces between DPDK library and DPDK applications. The system also supports crypto operations offload and ensures source code compatibility.

\item This paper conducts a series of evaluation under different network loads to estimate the performance difference between \sysname and future systems that support trusted I/O devices. Experimental results demonstrate \sysname's performance is within 6\% of the estimated performance of future systems with trusted I/O support.

\item This paper enhances an existing DPDK measurement tool to support end-to-end IPsec traffic measurement in the context of confidential VM environment.

\end{packeditemize}

\bheading{Paper outline.} The rest of the paper is organized as follows: \secref{sec:background} introduces background information about confidential VM and AMD SEV, as well as relevant network techniques; \secref{sec:motivation} and \secref{sec:conclusion} concludes the paper.

% In the paper, we aim to answer the following research questions:
% \begin{enumerate}[label=\textbf{Q\arabic*.}]
% \item \label{q1} What are the network performance bottlenecks of SEV-SNP enabled VMs?
% \item \label{q2} How is network I/O security ensured in SEV-SNP enabled VMs?
% \item \label{q3}
% Without a trusted I/O device, what is the performance limit of network I/O in SEV-SNP enabled VMs while ensuring security?
% \item \label{q4} What optimizations can Trusted I/O device bring?
% \end{enumerate}

==> x-motivation-backup.tex <==
\section{Identifying Network Performance Bottlenecks in SNP}
\label{sec:motivation}

% \mengjia{very confused. you already have implementation/evaluation results in this section, but you will only talk about DPDK implementation in TEE in the next section. From my perspective, this organization is a bit wired. Maybe we should discuss.}

\begin{figure}[t]
\centering
\includegraphics[width=0.75\columnwidth]{fig/combo_v3.pdf}
\caption{VirtIO network path.}
\label{fig:net_path}
\mengjia{is it possible to show the TEE-related overhead/path in this figure?}
\end{figure}

There are many factors that can slow down network performance in an SNP-enabled VM, including inherent factors from the virtualization environment and additional factors introduced by the security protection from SNP. The network performance bottlenecks in SNP may be caused by one or several of these factors. In this section, we first provide a comprehensive list of all factors and describe their consequences on network performance. We then conduct a series of motivated experiments to breakdown and identify the driving factors resulting in the performance bottlenecks in SNP.

\subsection{Factors from Virtualization}
While hardware-accelerated virtualization techniques, such as Intel VT~\cite{intel:2005:intel-vt} and AMD SVM~\cite{amd:2005:svm}, offer substantial performance improvements compared to software-based virtualization ~\cite{che:2010:synthetical,soriga:2013:comparison,deshane:2008:quantitative}, the performance of network applications running within VMs is still constrained by various factors inherent to virtualization, including overhead because of \textit{routing within the VM}, and \textit{routing within the host side} and \textit{I/O interrupt delay} due to emulated I/O devices. 

\bheading{Routing within the VM.} Network applications usually utilize the system call interface to inform the kernel and NIC about sending and receiving network packets. In a VM setup, such routing happens within the VM itself, which introduces in the form of internal context switches and the VM kernel's handling of packet routing and processing. Moreover, the kernel commonly relies on an interrupt-driven mechanism to notify the application about the packet status, which leads to potential delays and additional context switches.


\bheading{Emulated I/O devices.} One of the main reasons for the subpar network performance in virtualization environment is the use of emulated network devices~\cite{hajnoczi:2017:applying}. Instead of directly communicating with physical NICs, VMs rely on QEMU to emulate virtual NICs. VMs interact solely with these emulated NICs, and QEMU interprets and forwards their requests to the physical NICs. As shown in \figref{fig:net_path}, when VM's vCPU prepares to transmit outgoing network packets, it initiates a notification to the host side through kicking a shared "virtqueue" structure. This notification is typically accomplished using an \texttt{iowrite} instruction, which is intercepted by the hardware, triggering the corresponding \texttt{VMEXIT}. Subsequently, the KVM module within the host kernel notifies QEMU of this event, and QEMU conveys the corresponding network request to the physical NIC through a system call. Similarly, for incoming network packets, the I/O interrupt is not directly delivered to the VM but is injected into the corresponding vCPU by QEMU and KVM. During the next \texttt{VMRUN}, the vCPU can then jump to its internal IRQ handler. This configuration of emulated network cards allows a single NIC to be shared among multiple VMs and offer domain isolation, as the interaction with the physical NICs is handled by QEMU and the host kernel. However, such emulated network devices suffer significant overhead introduced by multiple levels of context switches between the VM, QEMU, and the host kernel (\textit{Routing within the host}), as well as the additional delays introduced by emulated I/O interrupts (\textit{Emulated I/O interrupt overhead}). 



\bheading{Other factors.} 
Some factors that could be configured by software, such as scheduling, cache locality, and multi-threading, which are highly software dependent, are excluded as in this section we focus on exploring general factors that infect all applications. Hardware capabilities, such as CPU frequency, NIC bandwidth, and NIC response time, are also excluded.  
In addition to that, Kernel page-table isolation (KPTI)~\cite{muller:2018:kpti} adopted during ring switch, which is designed to against speculative execution attacks could bring additional overhead. In our evaluation setup across the paper, the corresponding kernel configuration \texttt{CONFIG\_PAGE\_TABLE\_ISOLATION} is always set to \texttt{Y} in both host and guest OS. 

% \begin{figure}[t]
% \centering
% \begin{subfigure}[b]{0.95\columnwidth}
% \includegraphics[width=\textwidth]{fig/outpath_v2.pdf}
% \caption{Traditional cloud model.}
% \label{fig:outpath}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.85\columnwidth}
% \includegraphics[width=\textwidth]{fig/inpath_v2.pdf}
% \caption{Cloud model with TEE. }
% \label{fig:inpath}
% \end{subfigure}
% \caption{Virtio-net network path.}
% \end{figure}


\begin{table*}[t]
\setlength{\tabcolsep}{3pt}
\centering
%\tiny
\scriptsize
% \footnotesize
\scalebox{1}{

    \begin{tabular}{cl|c|c|c|c|c|c|c|c|c}
        \hline\hline
        &\textbf{\tabincell{c}{Overhead Description}}	&	\textbf{\tabincell{c}{non-TEE VM}}	&
        \textbf{\tabincell{c}{VM with \\SRIOV}}	&
        \textbf{\tabincell{c}{VM with \\DPDK}}	&
        \textbf{SEV VM}	&  \textbf{\tabincell{c}{SEV with \\ SRIOV}} &
	\textbf{\tabincell{c}{ES with\\ SRIOV}}		& \textbf{\tabincell{c}{SNP with\\ SRIOV}}& \textbf{\tabincell{c}{SNP with\\ DPDK}}& \textbf{\tabincell{c}{SNP with\\ TIO}}\\\hline
                \\[-7.5pt]
                
        \multicolumn{1}{c}{\multirow{4}{*}{\rotatebox{90}{\texttt{\textbf{Common}}}}}	& \multicolumn{1}{|l|}{\texttt{Routing within the VM}}	&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}	&	\color{LimeGreen}\textbf{N}	&	\color{Maroon}\textbf{Y} & \color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}		&	\color{Maroon}\textbf{Y}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	\\
        
        &\multicolumn{1}{|l|}{\texttt{Routing within the host}}	&	\color{Maroon}\textbf{Y}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	&	\color{Maroon}\textbf{Y} & \color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	\\
        
        &\multicolumn{1}{|l|}{\texttt{Emulated I/O interrupt}}	&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}	&	\color{LimeGreen}\textbf{N}	&	\color{Maroon}\textbf{Y} & \color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}		&	\color{Maroon}\textbf{Y}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	\\
        
        &\multicolumn{1}{|l|}{\texttt{Other factors}}	&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y} & \color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}		&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}	\\
        \hline 
        \\[-7pt]
        %\multicolumn{6}{l}{\textbf{ENCLU}} \\ \hline								
        \multicolumn{1}{c}{\multirow{5}{*}{\rotatebox{90}{\texttt{\textbf{SEV-only}}}}}	&\multicolumn{1}{|l|}{\texttt{Memory encryption overhead}}	&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y} &	\color{Maroon}\textbf{Y} &	\color{Maroon}\textbf{Y}		&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}	\\
        
        &\multicolumn{1}{|l|}{\texttt{Bounce buffer overhead}}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	&	\color{Maroon}\textbf{Y} &	\color{Maroon}\textbf{Y} &	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}	&	\color{LimeGreen}\textbf{N}	\\
        
        &\multicolumn{1}{|l|}{\texttt{VC handler overhead}}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	& \color{LimeGreen}\textbf{N} &	\color{Maroon}\textbf{Y}		&	\color{Maroon}\textbf{Y}	&	\color{LimeGreen}\textbf{N}$^*$	&	\color{LimeGreen}\textbf{N}$^*$	\\
        
        &\multicolumn{1}{|l|}{\texttt{VMEXIT check overhead}}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	& \color{LimeGreen}\textbf{N} &	\color{Maroon}\textbf{Y}		&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	&	\color{LimeGreen}\textbf{N}	\\
        
        &\multicolumn{1}{|l|}{\texttt{Ownership check overhead}}	&	\color{LimeGreen}\textbf{N${^-}$}	&	\color{LimeGreen}\textbf{N${^-}$}	&	\color{LimeGreen}\textbf{N${^-}$}	&	\color{LimeGreen}\textbf{N${^-}$}	& \color{LimeGreen}\textbf{N${^-}$} &	\color{LimeGreen}\textbf{N${^-}$}		&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}	&	\color{Maroon}\textbf{Y}	\\


	\hline\hline \\[-7pt] \multicolumn{11}{l}{\textbf{\hspace{9pt} Standardized Latency (5000 pps)}} \\\hline	

         &Mean latency   & >40x  & 1.00 (75.1 \textmu s)  & 0.37x & >40x & 1.01x& 1.17x & 1.16x & - & - \\
         &Median latency  & >40x & 1.00 (75.3 \textmu s)  & 0.36x & >40x & 1.02x & 1.18x & 1.13x &  - & -\\
         &p95 tail latency & >40x &1.00 (83.8 \textmu s)   & 0.33x & >40x & 1.00x & 1.20x & 1.18x  & - & - \\
         &p99 tail latency & >40x & 1.00 (123.6 \textmu s) & 0.31x & >40x & 0.78x& 0.94x& 2.19x & - & - \\
         
        \hline\hline 
    \end{tabular}
}
\vspace*{10pt}
\caption{\small Template. With DPDK means the VM is using DPDK to operate a SRIOV device. For standardized latency, the performance of ``VM with DPDK" is chosen as the standard, as it has the lowest overhead. * indicates that VC handler overheads due to scheduler or interrupt are mitigated. - indicates that the ownership check only happens before write access. [maybe change the memory encryption overhead for non-TEE VM]}
\label{tab:factors}
\end{table*}

\subsection{Factors from SNP}
Other than the common factors faced by virtualization, protections enabled by confidential VM (SEV, SEV-ES, and SEV-SNP) bring additional factors that downgrade the network performance. 

\bheading{Memory encryption overhead.} Confidential VMs ensure the security of data stored in memory by utilizing memory encryption achieved by on-chip AES engines. Each VM has its private or shared memory encryption keys, which are securely stored within the CPU, safeguarding them from malicious CSP. However, memory encryption also introduces overhead as confidential VMs need to perform decryption and encryption before memory read and write, which leads to additional overhead compared to non-TEE VMs.
It is worth mentioning that many server processors also employ memory encryption for the hypervisor as well, such as AMD Secure Memory Encryption~\cite{kaplan:2016:sevWpaper} and Intel Total Memory Encryption~\cite{intel:2017:tme} features. In such cases, all memory pages, including memory pages owned by the hypervisor and non-TEE VMs but excluding memory pages owned by confidential VMs or some hardware meta data, share the same encryption key and store encrypted data in the memory.

\bheading{Bounce buffer overhead.} In SEV environment, I/O operations such as DMA automatically utilize the memory encryption key of the hypervisor. As a result, I/O data can only be written to a shared region between the VM and the hypervisor. Consequently, prior to processing I/O data, the guest VM's kernel must copy the I/O data from this shared region to the VM's private memory. This memory copy mechanism in SEV leverages Linux's bounce buffer design, which is originally designed to resolve the limitation of devices supporting only 32-bit addresses. However, such bounce buffer solution introduces two potential overheads.
The first overhead stems from the actual process of data copying. The second overhead arises due to memory encryption or decryption during the copying process. Since the shared area and private memory are encrypted using different encryption keys (\eg, the VM's private memory uses the VM's encryption key, while the shared region uses the host's memory encryption key), the copying process may require the utilization of distinct keys for encrypting and decrypting memory.

\bheading{VC handler overhead.} 
To ensure the security of VM register backups during \texttt{VMEXIT}, AMD SEV-ES and SEV-SNP encrypt the stored register values. However, this encryption prevents direct observation of register values by the hypervisor for certain instructions like \texttt{CPUID} or \texttt{RDMSR}. To address this, AMD introduced the VMM Communication Exception (VC exception) to intercept and emulate these instructions. When an instruction requiring hypervisor emulation is executed, the hardware intercepts it and redirects control flow to a VC handler within the guest kernel. The VC handler stores the register values required for hypervisor emulation in a shared region before triggering a VMEXIT. After the hypervisor simulates the corresponding return values and resumes the VM, execution continues from the VC handler. The VC handler then copies the return values back to the corresponding registers and returns control to the program that triggered the VC exception. AMD has standardized this design and provided a communication protocol, including a comprehensive list of intercepted instructions~\cite{amd:2020:ghcb}.

Apparently, this design introduces additional overheads, including additional handler overhead within the VM as well as overhead caused by hypervisor emulation, both of which can highly impact I/O performance. It is important to note that the VC exceptions occur more frequently than expected. 
Frequent \textit{CPUID} calls are common during the boot period, and during runtime, operations such as obtaining the current timestamp using \texttt{RDTSC}, setting timer interrupts with \texttt{WRMSR} for CPU scheduling, and performing I/O port operations all trigger frequent VC events. 




\bheading{VMEXIT integrity check overhead.} In SEV-ES, additional integrity checks are implemented by the hardware during the VM-host world switch to prevent attackers from tampering with or replaying register backups. More specifically, during \texttt{VMEXIT}, the hardware measures the VM save area (VMSA), which is the data structure storing the register backups. When performing a sequential \texttt{VMRUN}, the hardware verifies that the VMSA remains consistent with the previous measurement. Such integrity check can result in a decrease in I/O performance when there are frequent VM-host world switches.



\bheading{Ownership check overhead.} In SEV-SNP, the integrity check during VMEXIT is removed because SEV-SNP introduces ownership check to protect memory page integrity. A new data structure called the Reverse Map Table (RMP table) is introduced to store the ownership of each memory page and restricts the hypervisor from tampering with the VMSA page. However, as a trade-off, during most memory accesses, the hardware needs to compare the current executor's permissions with the RMP table to determine if such access is allowed. This additional memory access check could also affect I/O performance.





\subsection{Unraveling the Key Factors Influencing Performance}
\bheading{Evaluation methodology.} 
\mengjia{I do not know what exactly "macro-level comparison" means. And it is too early to spend so much text for defensive argument.}
When investigating the primary factors that impact network performance in confidential VMs, we chose to conduct a macro-level comparison instead of a detailed breakdown of individual factors' time consumption. Undoubtedly, the most effective approach to analyze overhead factors is to break down the time spent on each factor by recording timestamps. However, collecting such timestamps is not straightforward in VM setting. It requires modifying the host kernel to record timestamps to record time spent in routing within the host side. And it also requires recording timestamps when routing happens inside the VM, either intercepting VM execution or modifying the VM kernel to directly read timestamps. Both options significantly slow down the VM's packet processing speed, thereby making the act of reading timestamps itself a significant influencing factor.

For example, when a non-TEE VM employs the \texttt{RDTSCP} instruction to read timestamps, it triggers the corresponding \texttt{VMEXIT}. In the settings of SEV-ES and SEV-SNP, a even more complex routing occurs, involving an application to VC handler, to hypervisor, back to VC handler, and back to the application. In a network connection with 5000 packets per second, such intricate routing can introduce challenges in accurately assessing the dominant factors impacting network performance. 
On the other hand, the advantage of adopting a macro-level approach is that it allows us to eliminate irrelevant factors. By ensuring that all VMs have the same kernel, the same capability, and run on the same CPU, we can compare the different overheads across various settings and evaluate the impact of each specific overhead. For instance, as illustrated in \tabref{tab:factors}, the only distinction between ``non-TEE VM with SRIOV" and ``SEV VM with SRIOV" is whether bounce buffer is present.
A noteworthy example is that we found the bounce buffer could introduce up to 8\% overhead at the beginning of our investigation when we recorded the overhead using timestamps. However, when directly comparing non-TEE with SRIOV (no bounce buffer) and SEV with SRIOV (with bounce buffer), their performance only differ by less than 3\%.



\bheading{Experimental setup.}
\label{sec:motivation:setup}
% a Netgear GS110TPv3 switch
Our experimental setup consists of a SNP-supported workstation and a desktop client. The SNP-supported workstation has an AMD EPYC 7313 16-Core Processor, 64GB DRAM, 1TB disk, an Intel I350 Gigabit NIC for internet connection, and an Intel 82599ES-based 10Gb NIC (Silicom PE210G2SPI9) for supporting DPDK and SRIOV. The desktop client has an Intel i5-12400F Processor, 32GB DRAM, 500GB disk, an Intel I219-V NIC for sharing internet with the workstation, and another Intel 82599ES-based 10Gb NIC for supporting DPDK and SRIOV. The two Intel 82599ES NICs are connected by a MokerLink 8 Port 10Gbps switch. The original host kernel (\texttt{sev-snp-iommu-avic\_5.19-rc6\_v4} branch), QEMU (\texttt{snp-v3} branch), and OVMF (\texttt{master} branch) were directly obtained from the \texttt{sev-snp-devel} branch (Commit: \texttt{fbd1d07628f8a2f0e29e9a1d09b1ac6fdcf69475}) in AMD SEV's official GitHub repository~\cite{amd:2023:github}. The desktop client simply runs an unmodified Ubuntu 22.04.1 LTS with kernel of \texttt{5.19.0-38-generic}.

The VMs were configured as 4-virtual CPUs (vCPUs), 8-GB memory, 30GB disk storage. The guest kernel used to support SNP feature is forked and built from the same repository and commit version as the host kernel. For ``non-TEE VM" and ``SEV VM" setup, the VMs use the default virtio-net-pci device suggested by AMD's official script used for launching SEV VM~\cite{amd:2023:github}. For all SRIOV and DPDK setup, one NIC's virtual function (VF) is directed assigned to the VM via QEMU PCI pass-through configuration.   
The network server applications running inside VM are two simple UDP echo servers. One of them uses normal socket APIs, and the other is only used in ``VM with DPDK" setup and is configured using DPDK APIs. On the client side, we reuse a client application from an existing open-sourced project that focuses on measuring tail latency~\cite{kaffes:2019:shinjuku}. We configure the packet rate for the client application to be 5000 packets per second (pps). All other configurations remain consistent across each setup.

% \begin{center}
% \minibox[frame, rule=1pt,pad=3pt]{
% \begin{minipage}[t]{0.95\columnwidth}
% \textbf{Observation:} Most TEE designs utilize a unprotected mode for CPU scheduling and utilize RTPM-only mode for securely backup registers. 
% \end{minipage}
% }
% \end{center}
\bheading{Result analysis.} The evaluation results are summarized in \tabref{tab:factors}, where we standardized all tail latencies based on the performance of ``non-TEE VM with SRIOV" as the benchmark. By comparing various VM configurations, we can derive some intriguing observations.

\begin{center}
\begin{minipage}[t]{1\columnwidth}
\begin{mdframed}
\textbf{Observation-1:}
Overhead due to routing within the VM and routing within the hypervisor are the two dominant factors that impact performance.
\end{mdframed}
\end{minipage}
\vspace{1pt}
\end{center}

\begin{center}
\begin{minipage}[t]{1\columnwidth}
\begin{mdframed}
\textbf{Observation-2:}
Overhead due to VC handler overhead is one key factor that impact performance for newly SEV-ES and SEV-SNP VMs.
\end{mdframed}
\end{minipage}
\vspace{1pt}
\end{center}

\begin{center}
\begin{minipage}[t]{1\columnwidth}
\begin{mdframed}
\textbf{Observation-3:}
While SNP adds additional ownership check during memory access, its performance surpasses that of ES. This could be attributed to the significant performance impact caused by the integrity check added in VMEXIT for ES.
\end{mdframed}
\end{minipage}
\vspace{1pt}
\end{center}


\begin{center}
\begin{minipage}[t]{1\columnwidth}
\begin{mdframed}
\textbf{Observation-4:}
Under the setting of encrypted memory, the bounce buffer is an overhead that cannot be bypassed. However, the impact of this overhead may be smaller than we previous thought.
\end{mdframed}
\end{minipage}
\vspace{1pt}
\end{center}

Although the bounce buffer may be affected by packet size and throughput, the overhead it introduces might be smaller than people expected. The impact of packet size and different transmission rates on the bounce buffer will be covered in the subsequent evaluation.

\bheading{Research vision.} This exploratory section identifies the practical network overhead that caused by various TEE constraints impose on a confidential VM. The results themselves are also highly insightful. It is revealed that the memory copy resulting from encrypted memory is not the decisive limiting factor for confidential VMs. This indicates that with the assistance of SR-IOV and DPDK, high-performance I/O can be achieved in confidential VMs even without relying on hardware-dependent trusted I/O devices. Motivated by this exciting finding, the upcoming sections will focus on securely implementing SR-IOV and DPDK within the confidential VM environment, and compare their performance and security with future trusted I/O devices. [This subsection is very important, need to repeat motivation here]
